SimpleShot: Revisiting Nearest-Neighbor Classification for Few-Shot Learning

Few-shot learners aim to recognize new object classes based on a small number of labeled training examples. To prevent overfitting, state-of-the-art few-shot learners use meta-learning on convolutional-network features and perform classification using a nearest-neighbor classifier. This paper studies the accuracy of nearest-neighbor baselines without meta-learning. Surprisingly, we find simple feature transformations suffice to obtain competitive few-shot learning accuracies. For example, we find that a nearest-neighbor classifier used in combination with mean-subtraction and L2-normalization outperforms prior results in three out of five settings on the miniImageNet dataset.

==> ecoc.tex <==
\section{Error-Correcting Output Codes}
\label{sec:ecoc}
\emph{Error-correcting output codes (ECOC)} are the application of error-correcting codes \cite{bose1960,hocquenghem59} to the output of machine learning algorithms \cite{dietterich95}. They were used in early deep networks \cite{sejnowski87} but have not been very popular in modern network architectures. The key idea of error-correcting output codes is to encode each class in a multi-classification problem using a binary code, and to train the machine learning model to predict the bits in this code. Predictions are performed by using the trained model to predict the binary code and \emph{decoding} the predicted code by finding the the most similar code across all classes. 

The binary code of a class can be designed in a variety of ways, for instance, to recover one-versus-one or one-versus-all classification \cite{dietterich95}, but we focus exclusively on random binary codes that have redundancies: we use much more than $\log_2(C)$ bits to encode a class in a classification problem with $C$ classes. The key advantage of the training models to predict such error-correcting output codes is that the class predictions are very robust to overfitting and that it is trivial to increase the set of classes the model can predict: adding a new class to be recognized amounts to finding the appropriate code for that class, which is straightforward. This makes error-correcting output codes particularly well-suited for few-shot learning problems.

\paragraph{Prediction with error-correcting output codes.} 
Assume we are given a real-valued input $\vx \in \R^D$ for which we need to predict a discrete class label $y \in \{0, 1, \dots, C\}$. We denote the error-correcting output code for class $y$ by $\vc^{(y)} \in \{0, 1\}^B$. Note that the code length, $B$, should be at least $\lceil \log_2(C) \rceil$ in order for the codes $\vc^{(y)}$ to successfully scatter all classes. In practice, we randomly sample all $CB$ bits in the error-correcting output codes uniformly at random; see Figure~\ref{fig:ecoc} for an illustration. 

Predictions are performed using a parametric model $f(\vx; \theta)$ with parameters $\theta$, for instance, a convolutional network. Given an input $\vx$, this model predicts a binary code $\vc \in \{0, 1\}^B$. Subsequently, the prediction $y$ is obtained by \emph{decoding} the code $\vc$, that is, by finding the error-correcting output code that is most similar in terms of Hamming distance:
\begin{equation}
y = \argmin_{y' \in \{1, 2, \dots, C\}} \sum_{b=1}^B \left| c_b - c^{(y')}_{b} \right|,
\label{eq:decoder}
\end{equation}
where $c_b$ denotes the $b$-th bit of binary code $\vc$.

\paragraph{Model training.} As is common practice in deep learning, the model $f(\vx; \theta)$ is trained using empirical risk minimization using a training set $\mathcal{D} = \{(\vx_1, y_1), (\vx_2, y_2), \dots, (\vx_N, y_N)\}$ that contains $N$ labeled training examples. Specifically, we minimize the empirical loss function that sums the discrepancy between the prediction $f(\vx_n; \theta)$ and the corresponding label $\vc^{(y_n)}$ over all $N$ training examples. In our study, the loss function is defined to be a sum of $B$ binary cross-entropy losses. Training is performed using a standard gradient-based optimizer. See section~\ref{sec:experiments} for details.

%\WLC{We trained with a two-stage method, learning a $C$-way classifier first and then learn with ECOC. Details are in the implementation details.}

\paragraph{Recognizing a new class.} In a one-shot learning, we aim to recognize a new class $C+1$ based on a single labeled example of that class, $\vx_{N+1}$. Presuming our error-correcting output codes contain sufficiently many bits, our problem formulation allows us to do this \emph{without having to change the model $f(\vx; \theta)$} in any way. Indeed, we can simply extend our decoder to consider the additional class using the error-correcting output code $\bc_{C+1} = f(\vx_{N+1}; \theta)$. In few-shot learning settings that provide $K$ labeled examples for the new class, we use a ``soft'' code instead that is given by $\vc_{C+1} = \frac{1}{K} \sum_{k=1}^K f(\vx_{N+k}; \theta)$; we use this soft code for the new class in the decoder in Equation~\ref{eq:decoder}.

\WLC{Currently we are using ${-1, 1}$ coding and perform cosine similarity, which is equivalent to Hamming distance in the one-shot case, but not the same in the multiple-shot one.}
